Concept-skill Transferability-based Data Selection for Large Vision-Language Models

Instruction tuning, or supervised finetuning on extensive task-specific data, is necessary for Large Vision-Language Models (LVLMs) to generalize well across a broad range of vision-language (VL) tasks. However, training on large VL datasets can become prohibitively expensive. In this work, we introduce COINCIDE, an effective and scalable data selection technique that uses a small model as a reference model to select visual instruction tuning data for efficient finetuning of a target LVLM, focusing on diversity and transferability. Specifically, we cluster the training data using internal activations from a small model, which identifies VL concept-skill compositions needed by a target LVLM. We then sample data from these diverse clusters by considering their density and transferability, or the ability to transfer well to other concept-skill compositions. This approach ensures the diversity of these compositions, which is vital for LVLM generalization. Extensive experiments demonstrate that COINCIDE achieves superior performance and data selection efficiency against 8 strong baselines on two distinct datasets: LLaVA-1.5 and Vision-Flan. Using only 20% of the LLaVA-1.5 dataset, COINCIDE achieves performance comparable to the LVLM finetuned on the whole dataset, with 70% reduction of the wall-clock running time. On the Vision-Flan dataset, our method achieves superior results with only 16.7% of the training data.

==> materials/supplement_curri_algo.tex <==
\begin{figure*}[t]
\begin{minipage}{\textwidth}
    \centering
    \begin{algorithm}[H]
        \caption{\small \ours+ Curriculum Learning Algorithm}
        \label{alg:curri_algo}
        \begin{algorithmic}[1]
            \small
            \REQUIRE $K$: the number of clusters, $\gamma$: exploration rate, $\mu$: moving average rate, $T$: the number of rounds $S$: the number of steps per round, $\mathcal{D}=\{\mathcal{D}_1,\ldots,\mathcal{D}_K\}$: Dataset for $K$ clusters, $f_\theta$: training model
            \INIT $R_i=0$, $\mathcal{L}_{i,\text{past}}=0$\;\;$i\!\in\!\{1,2,\ldots,K\}$
            \FOR{$t = 1,2,\ldots,T$}
                \STATE $p_i(t)\!=\!(1-\gamma)\frac{R_i}{\sum_{j=1}^{K}}+\frac{\gamma}{K}$,\;\;$i\!\in\!\{1,2,\ldots,K\}$ \COMMENTARR{Calculate cluster selection distribution at step $t$}
                \FOR{$s = 1,2,\ldots,S$}
                    \STATE $D_i\sim p(t)$ \COMMENTARR{Select cluster $i$ from the step $t$ distribution}
                    \STATE $B\sim D_i$ \COMMENTARR{Sample batch from cluster $i$}
                    \STATE $R_i \leftarrow (1 - \mu)R_i + \mu (\mathcal{L}_{i,\text{past}} - \mathcal{L}(f_\theta,B))$ \COMMENTARR{Upate reward of cluster $i$}
                    \STATE $\mathcal{L}_{i,\text{past}}=\mathcal{L}(f_\theta,B)$
                    \STATE $\theta \leftarrow \theta - \eta\nabla_{\theta}\mathcal{L}(f_\theta,B)$ \COMMENTARR{Update model parameters}
                \ENDFOR
            \ENDFOR
        \end{algorithmic}
    \end{algorithm}
\end{minipage}
\vspace{-0.2in}
\end{figure*}

==> materials/tables/5_transfer_larger.tex <==
\resizebox{1.0\textwidth}{!}{
    \renewcommand{\arraystretch}{1.4}
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{l c}
         \toprule
         {\textbf{Method}} & {\textbf{\relp (\%)}}\\
          \midrule
         Full-Finetune(13B) & 100\\
         \midrule
         Random & 94.0\\
         CLIP-Score & 90.7\\
         EL2N & 93.8\\
         Perplexity & 91.6\\
         SemDeDup & 91.9\\
         D2-Pruning & \underline{94.7}\\
         Self-Sup & 93.6\\
         Self-Filter & 92.2\\
         \cellcolor{gg}\ours (Ours) & \cellcolor{gg}\textbf{95.9}\\
         \bottomrule
    \end{tabular}
}
\label{tab:ablation_transfer_larger}


==> materials/tables/5_vision_flan_tive_compare.tex <==
\begin{table}[t]
    \tiny
    \vspace{-0.05in}
    \caption{\small Comparison with techniques specialized for VIT coreset selection. The top table shows our Vision-Flan experiment results with a 16.7\% sampling ratio. The bottom table shows the Vision-Flan results taken from TIVE~\citep{Liu2024tive}, marked with $^{\dagger}$, which finetunes LVLMs for two epochs with the same sampling ratio, evaluated on three benchmarks. \abl{This is different from our setting?? We need fair comparisons.} \jwl{The direct comparison was hard since (1) they finetuned the entire parameters in their experiments and (2) they trained the models for 2 epochs. However, in our setting, we apply the LoRA to the target LVLM models due to the GPU limit and train the models for 1 epoch. Hence, we tried to compare the percent point gain compared to the random baseline and emphasize that \ours does not require task label and gradient calculation. Plus, the task labels are not mentioned in the main text. Should we erase the "Task labels" column in the Table 3? I thought that not using the task label is beneficial to emphasize that we do data selection in cluster-level, not in dataset level or in task level - JWL} \abl{Does merging the tables make sense? If so, then this is fine but we need to explain more in the main text. The table caption is probably not a good place to introduce too much nuance. If this is not ok due to different definitions of 100\%, then I wonder if we need to include this table. We do not need to compare against preprints that are not peer reviewed. } \jwl{The merging seems to be inappropriate due to the different definition of the \relp as you mentioned. Or, we can add more details in the table as I modified below.} \abl{I think the best thing to do is to remove reference to TIVE. We do not have a strict time comparison, do we? All that qualitative rationales just sound weak without concrete evidence. Do not gift the reviewer a reason to reject you. } \jwl{I understand. Let's just remove it! We can make this table commented!} \abl{sounds good!}}  
    \vspace{-0.1in}
    \centering
    \resizebox{\linewidth}{!}{
        \renewcommand{\arraystretch}{1.1}
        \renewcommand{\tabcolsep}{5pt}
        \begin{tabular}{l c c c c c a}
             \toprule
             {\textbf{Method}} & {\textbf{Train}} & {\} {\textbf{Task}} & {\textbf{Gradient}} & {\textbf{Reference}} & {\textbf{\relp (\%)}}\\
             & {\textbf{labels}} & {\textbf{Calculation}} & {\textbf{Model Size}} & \\
             \midrule
             Full-Finetune &
             {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 100}\\
             \cmidrule{0-4}
              Random &
             {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 94.2}\\
                Self-Filter &
             {\small $\times$ } & {\small \color{crimson}$\circ$ } & {\scriptsize 7B} & {\scriptsize 87.6}\\
             Length$^{\dagger}$ & 
             {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 98.5} \\
             TIVE$^{\dagger}$ &
             {\small \color{crimson}$\circ$ } & {\small \color{crimson}$\circ$ } & {\scriptsize 7B} & {\scriptsize 99.2} \\
                \cellcolor{gg}\ours (Ours) &
             \cellcolor{gg}{\small $\times$ } & \cellcolor{gg}{\small $\times$ }  & \cellcolor{gg}{\scriptsize 2B} & \cellcolor{gg}{\scriptsize \textbf{101.0}}\\
             % \midrule
             %  \midrule
             % Full-Finetune$^{\dagger}$ &
             % {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 100} \\
             %  \cmidrule{0-4}
             % Random$^{\dagger}$ & 
             % {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 98.5} \\
             % Length$^{\dagger}$ & 
             % {\small $\times$ } & {\small $\times$ } & {\scriptsize 0} & {\scriptsize 98.5} \\
             % TIVE$^{\dagger}$ &
             % {\small \color{crimson}$\circ$ } & {\small \color{crimson}$\circ$ } & {\scriptsize 7B} & {\scriptsize 99.2} \\
             \bottomrule
        \end{tabular}
    }
    \label{tab:vision_flan_tive_compare}
    \vspace{-0.1in}
\end{table}

==> materials/tables/supplement_compare_to_tive.tex <==
\begin{table*}[t]
    \tiny
    \vspace{-0.05in}
    \caption{\small We finetune LVLMs with coresets collected from the Vision-Flan~\citep{Xu2024visionflan} dataset with \textbf{16.7\% sampling ratio} for a single epoch. In the top table, we compare with baseline methods on multimodal evaluation benchmarks referring to~\citep{Xu2024visionflan}. At the bottom of the table, we show the results from the TIVE~\citep{Liu2024tive} where it finetunes the LVLMs for two epochs with the same 16.7\% selection ratio. SEED-I~\citep{seed_i} is a multiple-choice evaluation benchmark that estimates image understanding capabilities.}
    \vspace{-0.1in}
    \centering
    \resizebox{0.9\textwidth}{!}{
        \renewcommand{\arraystretch}{1.1}
        \renewcommand{\tabcolsep}{5pt}
        \begin{tabular}{l c c c c c c c c a}
             \toprule
             {\textbf{Method}} & {\textbf{MMBench}} & {\textbf{MME}} & {\textbf{MM-Vet}} & {\textbf{POPE}} & {\textbf{SQA-I}} & {\textbf{SEED-I}} & {\textbf{Task}} & {\textbf{Gradient}} & {\textbf{\relp (\%)}}\\
             & {\textbf{en}} & & & & & & {\textbf{labels}} & {\textbf{Calculation}} & \\
             \midrule
             Full-Finetune &
             {\scriptsize 53.4} & {\scriptsize 1287.5} & {\scriptsize 25.6} & {\scriptsize 84.2} & {\scriptsize 61.3} & {\scriptsize - } & {\scriptsize $\times$ } & {\scriptsize $\times$ } & {\scriptsize 100}\\
             \cmidrule{0-9}
              Random &
             {\scriptsize 45.2} & {\scriptsize 1122.3} & {\scriptsize 26.1} & {\scriptsize 82.5} & {\scriptsize 60.9} & {\scriptsize - } & {\scriptsize $\times$ } & {\scriptsize $\times$ } & {\scriptsize 94.2}\\
                Self-Filter &
             {\scriptsize 28.6} & {\scriptsize 923.6} & {\scriptsize \textbf{30.0}} & {\scriptsize \textbf{83.3}} & {\scriptsize 59.3} & {\scriptsize - } & {\scriptsize $\times$ } & {\scriptsize \color{crimson}$\circ$ } & {\scriptsize 87.6}\\
                \cellcolor{gg}\ours (Ours) &
             \cellcolor{gg}{\scriptsize \textbf{56.7}} & \cellcolor{gg}{\scriptsize \textbf{1222.2}} & \cellcolor{gg}{\scriptsize 26.2} & \cellcolor{gg}{\scriptsize 81.9} & \cellcolor{gg}{\scriptsize \underline{63.8}} & \cellcolor{gg}{\scriptsize - } & \cellcolor{gg}{\scriptsize $\times$ } & \cellcolor{gg}{\scriptsize $\times$ } & \cellcolor{gg}{\scriptsize \textbf{101.0}}\\
             \midrule
             Full-Finetune & {\scriptsize - } & {\scriptsize - } & {\scriptsize - } & {\scriptsize 81.7} & {\scriptsize 65.6} & {\scriptsize 58.4} & {\scriptsize $\times$ } & {\scriptsize $\times$ } & {\scriptsize 100} \\
              \cmidrule{0-9}
             Random & {\scriptsize - } & {\scriptsize - } & {\scriptsize - } & {\scriptsize 81.1} & {\scriptsize 64.9} & {\scriptsize 56.8} & {\scriptsize $\times$ } & {\scriptsize $\times$ } & {\scriptsize 98.5} \\
             Length & {\scriptsize - } & {\scriptsize - } & {\scriptsize - } & {\scriptsize 81.8} & {\scriptsize 64.4} & {\scriptsize 56.8} & {\scriptsize $\times$ } & {\scriptsize $\times$ } & {\scriptsize 98.5} \\
             TIVE & {\scriptsize - } & {\scriptsize - } & {\scriptsize - } & {\scriptsize 81.5} & {\scriptsize 65.3} & {\scriptsize 57.4} & {\scriptsize \color{crimson}$\circ$ } & {\scriptsize \color{crimson}$\circ$ } & {\scriptsize 99.2} \\
             \bottomrule
        \end{tabular}
    }
    \label{tab:vision_flan_compare_to_tive}
    \vspace{-0.1in}
\end{table*}

==> materials/tables/supplement_curriculum.tex <==
\begin{table*}[t]
    \tiny
    \vspace{-0.1in}
    \caption{\small We perform a comparison with the curriculum learning baseline on various multimodal evaluation benchmarks. We finetune LVLMs with LLaVA-1.5~\citep{Liu2023llava15} dataset utilizing 20\% of the total steps for training. The best and the second best results are in \textbf{bold} and \underline{underlined}, respectively.}
    \vspace{-0.1in}
    \centering
    \resizebox{0.95\textwidth}{!}{
        \renewcommand{\arraystretch}{1.1}
        \renewcommand{\tabcolsep}{4pt}
        \begin{tabular}{l c c c c c c c cc c a}
             \toprule
             {\textbf{Method}} & {\textbf{VQAv2}} & {\textbf{GQA}} & {\textbf{VizWiz}} & {\textbf{SQA-I}} & {\textbf{TextVQA}} & {\textbf{POPE}} & {\textbf{MME}} & \multicolumn{2}{c}{\textbf{MMBench}} & {\textbf{LLaVA-}} & {\textbf{\relp (\%)}}\\
             & & & & & & & & {\textbf{en}} & {\textbf{cn}} & {\textbf{Bench}} & \\
             \midrule
             Full-Finetune &
             {\scriptsize 79.1} & {\scriptsize 63.0} & {\scriptsize 47.8} & {\scriptsize 68.4} & {\scriptsize 58.2} & {\scriptsize 86.4} & {\scriptsize 1476.9} & {\scriptsize 66.1} & {\scriptsize 58.9} & {\scriptsize 67.9} & {\scriptsize 100}\\
             \cmidrule{0-11}
              Random &
             {\scriptsize \underline{75.7}} & {\scriptsize \textbf{58.9}} & {\scriptsize \underline{44.3}} & {\scriptsize 68.5} & {\scriptsize \underline{55.3}} & {\scriptsize 84.7} & {\scriptsize \textbf{1483.0}} & {\scriptsize 62.2} & {\scriptsize 54.8} & {\scriptsize 65.0} & {\scriptsize \underline{95.8}}\\
              Skill-it~\citep{Chen2023skillit} &
             {\scriptsize 75.4} & {\scriptsize \underline{56.9}} & {\scriptsize 42.4} & {\scriptsize \underline{69.7}} & {\scriptsize \textbf{56.0}} & {\scriptsize \underline{84.9}} & {\scriptsize 1370.5} & {\scriptsize \underline{62.9}} & {\scriptsize \underline{55.2}} & {\scriptsize \textbf{68.2}} & {\scriptsize 95.3}\\
              COINCIDE+ (Ours) &
             {\scriptsize \textbf{75.8}} & {\scriptsize \underline{56.9}} & {\scriptsize \textbf{49.3}} & {\scriptsize \textbf{69.9}} & {\scriptsize 53.9} & {\scriptsize \textbf{86.0}} & {\scriptsize \underline{1470.0}} & {\scriptsize \textbf{64.0}} & {\scriptsize \textbf{56.4}} & {\scriptsize \underline{67.6}} & {\scriptsize \textbf{97.5}}\\
             \bottomrule
        \end{tabular}
    }
    \label{tab:curriculum}
    \vspace{-0.2in}
\end{table*}


==> materials/tables/supplement_effect_hyperparameter.tex <==
\begin{table}[t]
    \centering
    \tiny
    \caption{\textbf{Effect of hyperparameters.}}
    \vspace{-0.05in}
    \resizebox{0.65\linewidth}{!}{
    \renewcommand{\arraystretch}{1.2}
    \renewcommand{\tabcolsep}{5pt}
    \begin{tabular}{c c c}
         \toprule
         {$\bm{K}$} & {$\bm{\tau}$} & {\textbf{\relp (\%)}}\\
         \midrule
         7500 & 0.1 & {96.2}\\
         \textbf{10000} & \textbf{0.1} & \textbf{97.4}\\
         12500 & 0.1 & {97.1}\\
         10000 & 0.05 & {96.1}\\
         10000 & 0.2 & {96.8}\\
         \bottomrule
    \end{tabular}
}
\label{tab:effect_hyperparameter}
\end{table}


==> materials/tables/supplement_neuron_activation.tex <==
\begin{table}[t]
    \centering
    \tiny
    \caption{\small \textbf{Choice of multimodal neuron activation.}}
    \vspace{-0.05in}
    \resizebox{0.65\linewidth}{!}{
    \renewcommand{\arraystretch}{1.3}
    \renewcommand{\tabcolsep}{1.5pt}
    \begin{tabular}{l c}
         \toprule
         {\textbf{Neuron Activation}} & \relp (\%)\\
         \midrule
         Boolean & 95.7\\
         Last layer & 96.5\\
         Intermediate layers (Ours) & \textbf{97.4}\\
         \bottomrule
    \end{tabular}
}
\label{tab:neuron_activation}
\end{table}

